University as a Melting Pot: Long-term Effects of Internationalization

This paper provides the first evidence on the impact of exposure to international students on the long-term outcomes of native students. I combine unique survey and administrative data from the Netherlands covering one million students across three decades and employ an across-cohort design. I find that exposure to international students leads natives to (i) form social ties with non-natives, (ii) hold more positive attitudes towards migration and learning about other cultures, and (iii) seek opportunities abroad. Notably, I find precisely estimated zero effects on employment, income, entrepreneurship, and the share of international co-workers up to 25 years after university entry.

==> definitions.tex <==
\begin{tabular}{llllllll}
  \hline
  \hline \\[-2ex] 
\textbf{Panel A}: Employed & Nationality and high & Nationality & High school & Residency before & Country of & Parent's country \\ 
& school completion & & completion & enrollment & of birth & of birth \\ 
\hline
  \hline
International share &  &  &  &  &  &   \\ 
in 10\% points &  &  &  &  &  &   \\ 
         \hline
 Effect size &  &  &  &  &  &   \\ 
  N &  &  &  &  &  &   \\ 
False positive  &  &  &  &  &  &   \\ 
%False negative  & - & 0\% & 0.5\% & 0\% & 0\% & 0\% \\ 
      \hline
   \hline \\[-2ex] 
\textbf{Panel B}: Income percentile & &  &  &  &  &  &   \\ 
\hline
  \hline
International share &  &  &  &  &  &   \\ 
in 10\% points &  &  &  &  &  &   \\ 
         \hline
 Effect size &  &  &  &  &  &   \\ 
  N &  &  &  &  &  &   \\ 
False positive  &  &  &  &  &  &   \\ 
%False negative  & - & 0\% & 0.5\% & 0\% & 0\% & 0\% \\ 
      \hline
   \hline \\[-2ex] 
\textbf{Panel C}: Cohabited with a non-native & &  &  &  &  &  &   \\ 
\hline
  \hline
International share &  &  &  &  &  &   \\ 
in 10\% points &  &  &  &  &  &   \\ 
         \hline
 Effect size &  &  &  &  &  &   \\ 
  N &  &  &  &  &  &   \\ 
False positive  &  &  &  &  &  &   \\ 
%False negative  & - & 0\% & 0.5\% & 0\% & 0\% & 0\% \\ 
      \hline
   \hline \\[-2ex] 
\textbf{Panel D}: Married to a non-native  &  &  &  &  &  &   \\ 
\hline
  \hline
International share &  &  &  &  &  &   \\ 
in 10\% points &  &  &  &  &  &   \\ 
         \hline
 Effect size &  &  &  &  &  &   \\ 
  N &  &  &  &  &  &   \\ 
False positive  &  &  &  &  &  &   \\ 
%False negative  & - & 0\% & 0.5\% & 0\% & 0\% & 0\% \\ 
      \hline
   \hline
%\textbf{Panel B} Graduated & & & & & &  \\ 
%from a university &  &  &  & & &   \\ 
%\hline
%  \hline
%Share of int. stud. & & & & & &  \\ 
%in 10\% points & & & & & &  \\ 
%         \hline
%  Mean & & & & & &  \\ 
%  N & & & & & &  \\ 
%      \hline
%   \hline
\end{tabular}


==> eu.tex <==
\begin{tabular}{lllll}
  \hline
  \hline \\[-2ex] 
\textbf{Panel A} & Bachelor's degree  & Master's degree & Employed & Income percentile \\ 
 & completion & completion & 15 years post-enrollment & 15 years post-enrollment \\ 
\hline
  \hline
EU share & 0.002 & 0.000 & -0.001 & 0.002 \\ 
in 10\%-points & (0.003) & (0.004) & (0.001) & (0.002) \\ 
         \hline
  Mean & 0.754 & 0.366 & 0.951 & 0.713 \\ 
  Effect size & 0.3\% & -0.1\% & -0.1\% & 0.3\% \\ 
  Cohorts & 1988-2019 & 1988-2019 & 1988-2008 & 1988-2008 \\ 
  N & 1,039,289 & 1,039,289 & 542,043 & 542,043 \\
      \hline
   \hline \\[-2ex] 
\textbf{Panel B} & \multicolumn{2}{c}{Cohabited with a non-native} & \multicolumn{1}{l}{Married} & \multicolumn{1}{l}{Married to a }  \\ 
& \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{non-native} \\ 
 & 1-4 years & 5-15 years & 15 years post-enrollment &  15 years post-enrollment \\ 
\hline
  \hline
EU share & 0.007*** & 0.004*** & -0.003 & 0.001  \\ 
in 10\%-points & (0.001) & (0.001) & (0.004) & (0.001)  \\ 
         \hline
  Mean & 0.027 & 0.091 & 0.473 & 0.035 \\ 
  Effect size & 25.7\% & 4.7\% & -0.7\% & 2.9\% \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1989-2008 & 1989-2008 \\ 
  N & 967,331 & 602,894 & 588,915 & 588,915 \\ 
\hline
\hline \\[-2ex] 
\textbf{Panel C} & \multicolumn{2}{c}{Emigrated} & \multicolumn{2}{c}{Emigrated to a classmate's country}  \\ 
  & \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{2}{c}{N years post-enrollment}  \\ 
 & 1-4 years & 5-15 years & 1-4 years & 5-15 years \\ 
\hline
  \hline
EU share & 0.003*** & 0.007*** & 0.004*** & 0.014***  \\ 
in 10\%-points & (0.000) & (0.003) & (0.000) & (0.003)  \\ 
         \hline
  Mean & 0.005 & 0.100 & 0.005 & 0.014  \\ 
  Effect size & 14.2\% & 7.0\% & 85.2\% & 103.1\%  \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1990-2019 & 1989-2008 \\
  N & 970,187 & 606,675 & 967,264 & 582,285  \\ 
      \hline
   \hline
\end{tabular}



==> human_capital.tex <==
\begin{tabular}{lllll}
  \hline
  \hline \\[-2ex] 
   & Dropped out & Time to  & Bachelor's degree  & Master's degree \\ 
 & during 1st year & graduate & completion & completion  \\ 
\hline
  \hline
International share & -0.003 & -0.017 & 0.005* & 0.001 \\ 
in 10\%-points & (0.006) & (0.026) & (0.003) & (0.004)  \\ 
         \hline
  Mean & 0.267 & 4.613 & 0.754 & 0.366 \\ 
  Effect size & 0.1\% & -0.3\% & 0.7\% & 0.3\%  \\ 
%  Cohorts & 1988-2019 & 1988-2019 & 1988-2019 & 1988-2019  \\ 
  N & 1,039,289 & 783,842 & 1,039,289 & 1,039,289   \\
      \hline
   \hline
\end{tabular}



==> non_STEM.tex <==
\begin{tabular}{lllll}
  \hline
  \hline \\[-2ex] 
\textbf{Panel A} & Bachelor's degree  & Master's degree & Employed & Income percentile \\ 
 & completion & completion & 15 years post-enrollment & 15 years post-enrollment \\ 
\hline
  \hline
International share & 0.007** & -0.003 & -0.001 & 0.002 \\ 
in 10\%-points & (0.003) & (0.004) & (0.001) & (0.001) \\ 
         \hline
  Mean & 0.759 & 0.368 & 0.948 & 0.699 \\ 
  Cohorts & 1988-2019 & 1988-2019 & 1988-2008 & 1988-2008 \\ 
  N & 798,153 & 798,153 & 421,622 & 421,622 \\ 
      \hline
   \hline \\[-2ex] 
\textbf{Panel B} & \multicolumn{2}{c}{Cohabited with a non-native} & \multicolumn{1}{l}{Married} & \multicolumn{1}{l}{Married to a }  \\ 
& \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{non-native} \\ 
 & 1-4 years & 5-15 years & 15 years post-enrollment &  15 post-enrollment \\ 
\hline
  \hline
International share & 0.005*** & 0.004*** & -0.002 & 0.001** \\ 
in 10\%-points & (0.001) & (0.001) & (0.003) & (0.001) \\ 
         \hline
  Mean & 0.028 & 0.087 & 0.478 & 0.033 \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1989-2008 & 1989-2008 \\ 
  N & 743,404 & 467,356 & 457,603 & 457,603 \\ 
\hline
\hline \\[-2ex] 
\textbf{Panel C} & \multicolumn{2}{c}{Emigrated} & \multicolumn{2}{c}{Emigrated to a classmate's country}  \\ 
  & \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{2}{c}{N years post-enrollment}  \\ 
 & 1-4 years & 5-15 years & 1-4 years & 5-15 years \\ 
\hline
  \hline
International share & 0.003*** & 0.009*** & 0.004*** & 0.013*** \\ 
in 10\%-points & (0.000) & (0.002) & (0.000) & (0.002) \\ 
         \hline
  Mean & 0.021 & 0.096 & 0.005 & 0.015 \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1990-2019 & 1989-2008 \\
  N & 745,711 & 470,225 & 743,429 & 453,224 \\ 
      \hline
   \hline
\end{tabular}



==> non_eu.tex <==
\begin{tabular}{lllll}
  \hline
  \hline \\[-2ex] 
\textbf{Panel A} & Bachelor's degree  & Master's degree & Employed & Income percentile \\ 
 & completion & completion & 15 years post-enrollment & 15 years post-enrollment \\ 
\hline
  \hline
Non-EU share & 0.014* & 0.002 & -0.004 & -0.001 \\ 
in 10\%-points & (0.008) & (0.021) & (0.004) & (0.005) \\ 
         \hline
  Mean & 0.754 & 0.366 & 0.951 & 0.713 \\ 
  Effect size & 1.8\% & 0.5\% & -0.4\% & -0.2\% \\ 
  Cohorts & 1988-2019 & 1988-2019 & 1988-2008 & 1988-2008 \\ 
  N & 1,039,289 & 1,039,289 & 542,043 & 542,043 \\
      \hline
   \hline \\[-2ex] 
\textbf{Panel B} & \multicolumn{2}{c}{Cohabited with a non-native} & \multicolumn{1}{l}{Married} & \multicolumn{1}{l}{Married to a }  \\ 
& \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{non-native} \\ 
 & 1-4 years & 5-15 years & 15 years post-enrollment &  15 years post-enrollment \\ 
\hline
  \hline
Non-EU share & 0.007*** & 0.002 & -0.001 & 0.003  \\ 
in 10\%-points & (0.002) & (0.004) & (0.010) & (0.003)  \\ 
         \hline
  Mean & 0.027 & 0.091 & 0.473 & 0.035 \\ 
  Effect size & 24.9\% & 2.4\% & -0.2\% & 7.7\% \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1989-2008 & 1989-2008 \\ 
  N & 967,331 & 602,894 & 588,915 & 588,915 \\ 
\hline
\hline \\[-2ex] 
\textbf{Panel C} & \multicolumn{2}{c}{Emigrated} & \multicolumn{2}{c}{Emigrated to a classmate's country}  \\ 
  & \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{2}{c}{N years post-enrollment}  \\ 
 & 1-4 years & 5-15 years & 1-4 years & 5-15 years \\ 
\hline
  \hline
Non-EU share & 0.005*** & 0.001 & 0.007*** & 0.030***  \\ 
in 10\%-points & (0.002) & (0.006) & (0.001) & (0.007)  \\ 
         \hline
  Mean & 0.005 & 0.100 & 0.005 & 0.014  \\ 
  Effect size & 25.5\% & 1.5\% & 150.0\% & 220.4\%  \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1990-2019 & 1989-2008 \\
  N & 970,187 & 606,675 & 967,264 & 582,285  \\ 
      \hline
   \hline
\end{tabular}



==> results_survey.tex <==
\begin{tabular}{p{14cm} llllll}
  \hline
  \hline \\[-2ex]  
  & Coefficient & s.e. & Sharpened & Mean & Effect size & N  \\ 
  & & & $q$-value & & &   \\ 
  \hline
  \hline \\[-2ex]  
   1. Have you donated money to an organization for humanitarian aid, human rights, minorities or migrants? (0 - no, 1 - yes) & 0.106*** & (0.029) & [0.004] & 0.297 & 35.7\% & 1,237 \\[4ex]  
   2. Do you agree that people of foreign origin who legally reside in the Netherlands should be entitled to the same social security as Dutch citizens? (1 - fully disagree, 5 - fully agree) & 0.236** & (0.095) & [0.027] & 3.534 & 6.2\% & 1,185 \\[4ex] 
   3. Do you agree that it does not help a neighborhood if many people of foreign origin or descent move in? (1 - fully disagree, 5 - fully agree) & -0.135** & (0.063) & [0.049] & 3.455 & -4.1\% & 1,185 \\[4ex] 
   4. Where would you place yourself on a scale from 1 to 5, where 1 means that European unification has already gone too far and 5 means that it should go further? & 0.247*** & (0.069) & [0.004] & 1.649 & 11.5\% & 1,185 \\[4ex]
  \hline
  \hline
\end{tabular}


==> robustness_3.tex <==
\begin{tabular}{llllllllllll}
  \hline
  \hline \\[-2ex] 
\textbf{Panel A}: Married & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) \\ 
15 years post-enrollment & & & & & & & & & & & \\
\hline
  \hline
International share  & -0.002 & -0.002 & -0.002 & -0.002 & -0.001 & -0.001 & 0.000 & -0.002 & -0.002 & -0.002 & -0.002 \\
in 10\%-points  & (0.003) & (0.003) & (0.003) & (0.003) & (0.003) & (0.002) & (0.002) & (0.003) & (0.003) & (0.003) & (0.003) \\
  \hline
  %$R^2$  & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 & 0.01 & 0.02 & 0.01 & 0.01 & 0.01 & 0.02 \\ 
  N & 588,915 & 588,915 & 588,915 & 588,915 & 588,915 & 588,915 & 588,915 & 619,828 & 598,792 & 631,993 & 631,993 \\
  \hline
  \hline \\[-2ex] 
\textbf{Panel B}: Married to a non-native & & & & & & & & & & & \\
15 years post-enrollment & & & & & & & & & & & \\
\hline
  \hline
International share & 0.001** & 0.001** & 0.001** & 0.001** & 0.001* & 0.001** & 0.002** & 0.002** & 0.001* & 0.002** & 0.002** \\ 
in 10\%-points & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) & (0.001) \\
  \hline
  %$R^2$ & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 \\
  N & 588,915 & 588,915 & 588,915 & 588,915 & 588,915 & 588,915 & 588,915 & 619,828 & 598,792 & 631,993 & 631,993 \\
  \hline
  \hline \\[-2ex] 
\textbf{Panel C}: Emigrated & & & & & & & & & & & \\
1-4 years post-enrollment & & & & & & & & & & & \\
\hline
  \hline
International share & 0.003*** & 0.003*** & 0.003*** & 0.002*** & 0.003*** & 0.003*** & 0.003*** & 0.005*** & 0.003*** & 0.005*** & 0.004*** \\ 
in 10\%-points & (0.000) & (0.000) & (0.000) & (0.000) & (0.000) & (0.000) & (0.000) & (0.001) & (0.000) & (0.001) & (0.001) \\
  \hline
  %$R^2$ & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.02 & 0.03 & 0.03 & 0.02 & 0.03 & 0.03 \\
  N & 970,187 & 970,187 & 970,187 & 970,187 & 970,187 & 970,187 & 970,187 & 1,027,089 & 982,276 & 1,042,564 & 1,042,564 \\
  \hline
  \hline \\[-2ex] 
\textbf{Panel D}: Emigrated  & & & & & & & & & & & \\
5-15 years post-enrollment & & & & & & & & & & & \\
\hline
  \hline
International share & 0.007*** & 0.007*** & 0.007*** & 0.008*** & 0.007*** & 0.007*** & 0.007*** & 0.009*** & 0.007*** & 0.009***  & 0.009*** \\ 
in 10\%-points & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) \\
  \hline
  %$R^2$ & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 & 0.07 \\
  N & 606,675 & 606,675 & 606,675 & 606,675 & 606,675 & 606,675 & 606,675 & 641,901 & 616,666 & 654,422 & 654,422 \\
    \hline
  \hline \\[-2ex]
\textbf{Panel E}: Emigrated to a classmate's country & & & & & & & & & & & \\
1-4 years post-enrollment & & & & & & & & & & & \\
\hline
  \hline
International share & 0.003*** & 0.003*** & 0.003*** & 0.003*** & 0.003*** & 0.003*** & 0.003*** & 0.005*** & 0.003*** & 0.005*** & 0.005*** \\ 
in 10\%-points & (0.000) & (0.000) & (0.000) & (0.000) & (0.000) & (0.000) & (0.000) & (0.001) & (0.000) & (0.001) & (0.001) \\
  \hline
  %$R^2$ & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 & 0.04 \\
  N & 967,264 & 967,264 & 967,264 & 967,264 & 967,264 & 967,264 & 967,264 & 1,022,750 & 979,275 & 1,038,053 & 1,038,053 \\
  \hline
  \hline \\[-2ex] 
\textbf{Panel F}: Emigrated to a classmate's country & & & & & & & & & & & \\
5-15 years post-enrollment & & & & & & & & & & & \\
\hline
  \hline
International share & 0.013*** & 0.013*** & 0.013*** & 0.013*** & 0.013*** & 0.013*** & 0.013*** & 0.015*** & 0.013*** & 0.015*** & 0.015*** \\ 
in 10\%-points & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) & (0.002) \\
  \hline
  %$R^2$ & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 & 0.06 \\
  N & 582,285 & 582,285 & 582,285 & 582,285 & 582,285 & 582,285 & 582,285 & 612,869 & 592,110 & 624,952 & 624,952 \\
  \hline
  \hline \\[-2ex] 
  \textit{Controls} & & & & & & & & & & & \\
  ~~Field specific linear time trend & & \checkmark & & & & & \checkmark & & & & \checkmark \\
  ~~Field specific quadratic time trend & & & \checkmark & & & & \checkmark & & & & \checkmark \\
  ~~Program size & & & & \checkmark & & & \checkmark & & & & \checkmark \\
  ~~Individual characteristics & & & & & \checkmark & & \checkmark & & & & \checkmark \\
  ~~Peer characteristics & & & & & & \checkmark & \checkmark & & & & \checkmark \\
  \textit{Sample} & & & & & & & & & & & \\
  ~~First-generation immigrants & & & & & & & & \checkmark & & \checkmark & \checkmark \\
  ~~Students older than 30 at enrollment & & & & & & & &  & \checkmark & \checkmark & \checkmark \\
      \hline
   \hline
\end{tabular}



==> sex.tex <==
\begin{tabular}{lllll}
  \hline
  \hline \\[-2ex] 
\textbf{Panel A} & Bachelor's degree  & Master's degree & Employed & Income percentile \\ 
 & completion & completion & 15 years post-enrollment & 15 years post-enrollment \\ 
\hline
  \hline
International share & 0.006** & 0.000 & -0.001 & 0.001 \\ 
in 10\%-points  & (0.003) & (0.006) & (0.001) & (0.002)  \\ 
x $\mathds{1}$ [Female = 1] & -0.002 & 0.001 & 0.001  & 0.002 \\ 
  & (0.003) & (0.005) & (0.002) & (0.003) \\ 
         \hline
  Mean for males & 0.715 & 0.343 & 0.962 & 0.773 \\ 
  Mean for females & 0.793 & 0.389 & 0.939 & 0.650 \\ 
  Cohorts & 1988-2019 & 1988-2019 & 1988-2008 & 1988-2008 \\ 
  N  & 1,039,289 & 1,039,289 & 542,043 & 542,043 \\ 
      \hline
   \hline \\[-2ex] 
\textbf{Panel B} & \multicolumn{2}{c}{Cohabited with a non-native} & \multicolumn{1}{l}{Married} & \multicolumn{1}{l}{Married to a }  \\ 
& \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{non-native} \\ 
 & 1-4 years & 5-15 years & 15 years post-enrollment &  15 post-enrollment \\ 
\hline
  \hline
International share & 0.006*** & 0.005*** & -0.001 & 0.002*  \\ 
in 10\%-points & (0.001) & (0.001) & (0.004) & (0.001)  \\ 
x $\mathds{1}$ [Female = 1] & -0.001 & -0.003 & -0.002 & -0.001  \\ 
  & (0.001) & (0.002) & (0.004) & (0.001)  \\ 
         \hline
  Mean for males & 0.026 & 0.106 & 0.447 & 0.044  \\ 
  Mean for females & 0.028 & 0.077 & 0.500  & 0.026 \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1990-2008 & 1989-2008 \\ 
  N  & 967,331 & 602,894 & 588,915 & 588,915 \\ 
\hline
\hline \\[-2ex] 
\textbf{Panel C} & \multicolumn{2}{c}{Emigrated} & \multicolumn{2}{c}{Emigrated to a classmate's country}  \\ 
  & \multicolumn{2}{c}{N years post-enrollment} & \multicolumn{2}{c}{N years post-enrollment}  \\ 
 & 1-4 years & 5-15 years & 1-4 years & 5-15 years \\ 
\hline
  \hline
International share & 0.003*** & 0.008***  & 0.003*** & 0.015***  \\ 
in 10\%-points  & (0.001) & (0.002) & (0.000) & (0.002)  \\ 
x $\mathds{1}$ [Female = 1]  & 0.000 & -0.001  & 0.000 & -0.005*** \\ 
  & (0.001) & (0.003) & (0.000) & (0.001)  \\ 
         \hline
  Mean for males & 0.019 & 0.106 & 0.004 & 0.014  \\ 
  Mean for females & 0.020 & 0.094 & 0.005 & 0.013  \\ 
  Cohorts & 1990-2019 & 1989-2008 & 1990-2019 & 1989-2008 \\
  N  & 970,187 & 606,675 & 967,264 & 582,285  \\ 
      \hline
   \hline
\end{tabular}


